Optimizing Explanations by Network Canonization and Hyperparameter Search

Explainable AI (XAI) is slowly becoming a key component for many AI applications. Rule-based and modified backpropagation XAI approaches however often face challenges when being applied to modern model architectures including innovative layer building blocks, which is caused by two reasons. Firstly, the high flexibility of rule-based XAI methods leads to numerous potential parameterizations. Secondly, many XAI methods break the implementation-invariance axiom because they struggle with certain model components, e.g., BatchNorm layers. The latter can be addressed with model canonization, which is the process of re-structuring the model to disregard problematic components without changing the underlying function. While model canonization is straightforward for simple architectures (e.g., VGG, ResNet), it can be challenging for more complex and highly interconnected models (e.g., DenseNet). Moreover, there is only little quantifiable evidence that model canonization is beneficial for XAI. In this work, we propose canonizations for currently relevant model blocks applicable to popular deep neural network architectures,including VGG, ResNet, EfficientNet, DenseNets, as well as Relation Networks. We further suggest a XAI evaluation framework with which we quantify and compare the effect sof model canonization for various XAI methods in image classification tasks on the Pascal-VOC and ILSVRC2017 datasets, as well as for Visual Question Answering using CLEVR-XAI. Moreover, addressing the former issue outlined above, we demonstrate how our evaluation framework can be applied to perform hyperparameter search for XAI methods to optimize the quality of explanations.

==> coco_experiments_section.tex <==

\section{MS-Coco 2014 Experiments}
\label{sec:experiments_coco}
\subsection{Classes}
\label{app:sec:imagenet_classes}
In our experiments we considered the following 10 classes that were picked randomly:

\emph{``person'',  ``bear'',  ``umbrella'',  ``suitcase'',  ``kite'', ``surf board'',  ``wine glass'',  ``carrot'',  ``toilet'',  ``tv''}.

\subsection{Dataset Description}
The MS Coco 2014 dataset has images from 80 categories, including about 83000 training and 4100 validation samples with segmentation mask annotations, along with a private test set. This dataset is also much more diverse compared to ILSVRC2017 and does not suffer from the center-bias.

\subsection{Models}  We evaluate explanations on VGG-16, ResNet-18, EfficientNet-B0 and DenseNet-121. Similar to the Pascal VOC dataset, we fine tuned models using pre-trained models from the PyTorch model zoo. We use stochastic gradient descent as the learning algorithm. We use sum of binary cross entropy losses as the loss, and train the networks for until convergence. We opted to use a smaller learning rate for pretrained parameters. We excluded hard examples while training and during the evaluations.

\subsection{Results} The results are shown in Tables~\ref{tab:vgg_COCO}~-~\ref{tab:densenet_COCO}. The results suggest that for MS COCO, canonization helps explanations in all metrics, except for Faithfulness and Randomization metrics where results are not consistent across model architectures.
\begin{table*}[ht]
    \centering
    \include{results/COCO/vgg_COCO}
    \caption{\label{tab:vgg_COCO}Results for MS Coco XAI evaluation with VGG-16. Arrows indicate whether high ($\uparrow$) or low ($\downarrow$) are better. Best results are shown in bold.}
\end{table*}

\begin{table*}[ht]
    \centering
    \include{results/COCO/resnet_COCO}
    \caption{\label{tab:resnet_COCO}Results for MS Coco XAI evaluation with ResNet-18. Arrows indicate whether high ($\uparrow$) or low ($\downarrow$) are better. Best results are shown in bold.}
\end{table*}

\begin{table*}[ht]
    \centering
    \include{results/COCO/efficientnet_COCO}
    \caption{\label{tab:efficientnet_COCO}Results for MS Coco XAI evaluation with EfficientNet-B0. Arrows indicate whether high ($\uparrow$) or low ($\downarrow$) are better. Best results are shown in bold.}
 \end{table*}


\begin{table*}[ht]
    \centering
    \include{results/COCO/densenet_COCO}
    \caption{\label{tab:densenet_COCO}Results for MS Coco XAI evaluation with DenseNet-121. Arrows indicate whether high ($\uparrow$) or low ($\downarrow$) are better. Best results are shown in bold.}
\end{table*}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> results/COCO/densenet_COCO.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
\begin{tabular}{l||cc|cccc|cccc|cc|cccc}
\toprule
{} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
{} & \multicolumn{2}{c|}{$\uparrow$\ Spars.} & \multicolumn{2}{c}{$\uparrow$ Corr.} & \multicolumn{2}{c|}{$\uparrow$ AoPC} & \multicolumn{2}{c}{$\uparrow$ RMA} & \multicolumn{2}{c|}{$\uparrow$ RRA} & \multicolumn{2}{c|}{$\downarrow$ Logit} & \multicolumn{2}{c}{$\downarrow$ Avg. Sens.} & \multicolumn{2}{c}{$\downarrow$ Max Sens.} \\
canonized &         no &   yes &           no &   yes &    no &   yes &           no &   yes &    no &   yes &      no &   yes &         no &   yes &        no &   yes \\
\midrule
EB  &  \textbf{0.65}  &  0.58  &  0.01  &  \textbf{0.04}  &  0.13  &  \textbf{0.29}  &  0.22  &  \textbf{0.29}  &  0.25  &  \textbf{0.39}  &  0.85  &  \textbf{0.78}  &  0.57  &  \textbf{0.20}  &  1.02  &  \textbf{0.23}\\
LRP-$\varepsilon$+  &  0.64  &  0.64  &  0.01  &  \textbf{0.03}  &  0.17  &  \textbf{0.31}  &  0.25  &  \textbf{0.32}  &  0.29  &  \textbf{0.40}  &  0.61  &  \textbf{0.48}  &  0.62  &  \textbf{0.47}  &  1.14  &  \textbf{0.78}\\
LRP-$\alpha2\beta1$  &  \textbf{0.82}  &  0.74  &  0.00  &  \textbf{0.01}  &  0.16  &  \textbf{0.31} &  0.24  &  \textbf{0.34}  &  0.25  &  \textbf{0.37}  &  0.48  &  \textbf{0.38}  &  0.62  &  \textbf{0.50}  &  1.14  &  \textbf{0.77}\\
\bottomrule
\end{tabular}
}


==> results/COCO/efficientnet_COCO.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
\begin{tabular}{l||cc|cccc|cccc|cc|cccc}
\toprule
{} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
{} & \multicolumn{2}{c|}{$\uparrow$\ Spars.} & \multicolumn{2}{c}{$\uparrow$ Corr.} & \multicolumn{2}{c|}{$\uparrow$ AoPC} & \multicolumn{2}{c}{$\uparrow$ RMA} & \multicolumn{2}{c|}{$\uparrow$ RRA} & \multicolumn{2}{c|}{$\downarrow$ Logit} & \multicolumn{2}{c}{$\downarrow$ Avg. Sens.} & \multicolumn{2}{c}{$\downarrow$ Max Sens.} \\
canonized &         no &   yes &           no &   yes &    no &   yes &           no &   yes &    no &   yes &      no &   yes &         no &   yes &        no &   yes \\
\midrule
EB  &  0.56  &  \textbf{0.70}  &  0.00  &  0.0  &  0.17  &  \textbf{0.20}  &  0.23  &  \textbf{0.30}  &  0.28  &  \textbf{0.35}  &  1.00  &  \textbf{0.99}  &  0.40  &  \textbf{0.35}  &  0.47  &  \textbf{0.39}\\
LRP-$\alpha2\beta1$  &  0.73  &  \textbf{0.77}  &  0.00  &  0.0  &  \textbf{0.21}  &  0.11  &  \textbf{0.31}  &  0.30  &  \textbf{0.34}  &  0.31  &  0.64  &  \textbf{0.54}  &  0.56  &  0.56  &  0.77  &  0.77\\
LRP-$\varepsilon$+  &  0.53  &  \textbf{0.73}  &  \textbf{0.01}  &  0.0  &  0.22 & 0.22  &  0.27  &  \textbf{0.34}  &  0.38  &  \textbf{0.39}  &  \textbf{0.61}  &  0.67  &  \textbf{0.40}  &  0.43  &  \textbf{0.70}  &  0.71\\
\bottomrule
\end{tabular}

}


==> results/COCO/resnet_COCO.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
\begin{tabular}{l||cc|cccc|cccc|cc|cccc}
\toprule
{} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
{} & \multicolumn{2}{c|}{$\uparrow$\ Spars.} & \multicolumn{2}{c}{$\uparrow$ Corr.} & \multicolumn{2}{c|}{$\uparrow$ AoPC} & \multicolumn{2}{c}{$\uparrow$ RMA} & \multicolumn{2}{c|}{$\uparrow$ RRA} & \multicolumn{2}{c|}{$\downarrow$ Logit} & \multicolumn{2}{c}{$\downarrow$ Avg. Sens.} & \multicolumn{2}{c}{$\downarrow$ Max Sens.} \\
canonized &         no &   yes &           no &   yes &    no &   yes &           no &   yes &    no &   yes &      no &   yes &         no &   yes &        no &   yes \\
\midrule
EB  &  0.51  &  \textbf{0.55}  &  0.03  &  0.03  & \textbf{0.23}  &  0.22  &  0.25  &  \textbf{0.26}  &  0.33  &  0.33  &  \textbf{0.97}  &  0.98  &  0.16  &  \textbf{0.15}  &  0.17  &  \textbf{0.16}\\
LRP-$\alpha2\beta1$  &  0.69  &  \textbf{0.76}  &  0.02  &  0.02  &  0.25  &  0.25  &  0.28  &  \textbf{0.32}  &  0.32  &  \textbf{0.34}  &  0.69  &  \textbf{0.67}  &  \textbf{0.45}  &  0.46  &  0.73  &  0.73\\
LRP-$\varepsilon$+  &  0.54  &  \textbf{0.60}  &  0.03  &  0.03  & 0.23  &  \textbf{0.24}  &  0.25  &  \textbf{0.27}  &  0.33  &  \textbf{0.34}  &  0.73  &  0.73  &  0.42  &  \textbf{0.41}  &  0.72  &  \textbf{0.71}\\
\bottomrule
\end{tabular}

}


==> results/COCO/vgg_COCO.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
\begin{tabular}{l||cc|cccc|cccc|cc|cccc}
\toprule
{} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
{} & \multicolumn{2}{c|}{$\uparrow$\ Spars.} & \multicolumn{2}{c}{$\uparrow$ Corr.} & \multicolumn{2}{c|}{$\uparrow$ AoPC} & \multicolumn{2}{c}{$\uparrow$ RMA} & \multicolumn{2}{c|}{$\uparrow$ RRA} & \multicolumn{2}{c|}{$\downarrow$ Logit} & \multicolumn{2}{c}{$\downarrow$ Avg. Sens.} & \multicolumn{2}{c}{$\downarrow$ Max Sens.} \\
canonized &         no &   yes &           no &   yes &    no &   yes &           no &   yes &    no &   yes &      no &   yes &         no &   yes &        no &   yes \\
\midrule
EB  &  0.58  &  0.58  &  0.03  &  0.03  &  0.25  &  0.25  &  0.26  &  0.26  &  0.32  &  \textbf{0.33}  &  1.00  &  1.00  &  0.23  &  \textbf{0.19}  &  0.25  &  \textbf{0.21}\\
LRP-$\alpha2\beta1$  &  0.74  &  \textbf{0.86}  &  \textbf{0.03}  &  0.01  &  0.32  &  \textbf{0.35}  &  0.32  &  \textbf{0.39}  &  0.35  &  \textbf{0.37}  &  \textbf{0.53}  &  0.61  &  0.52  &  0.52  &  0.79  &  0.79\\
LRP-$\varepsilon$+  &  0.58  &  \textbf{0.66}  &  0.05  &  0.05  & 0.29  &  \textbf{0.32}  &  0.29  &  \textbf{0.34}  &  0.41  &  \textbf{0.42}  &  0.50  &  \textbf{0.47}  &  0.50  &  0.50  &  0.79  &  \textbf{0.78}\\
\bottomrule
\end{tabular}

}


==> results/VOC/d121_old_results.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                \textbf{0.64} &  0.51 &                  0.0 &  \textbf{0.02} &                  \textbf{0.44} &  0.34 &         0.21 &  \textbf{0.28} &         0.24 &  \textbf{0.37} &          \textbf{0.72} &  0.91 &               0.59 &  \textbf{0.19} &           1.10 &  \textbf{0.20} \\
LRP-$\varepsilon$+&               \textbf{ 0.67} &  0.58 &                  0.0 &  0.00 &                  \textbf{0.22} &  0.19 &         \textbf{0.25} &  0.24 &         0.28 &  \textbf{0.29} &          \textbf{0.36} &  0.42 &               0.63 & \textbf{0.47} &           1.00 &  \textbf{0.59} \\
LRP-$\alpha2\beta1$ &                \textbf{0.83} &  0.66 &                  0.0 &  0.00 &                  \textbf{0.34} &  0.31 &         0.24 &  \textbf{0.26} &         0.25 &  \textbf{0.27} &          0.38 &  \textbf{0.27} &               0.64 &  \textbf{0.51} &           1.09 &  \textbf{0.61} \\
\bottomrule
\end{tabular}}

==> results/VOC/d161_old.tex <==
\resizebox{\textwidth}{!}{ 
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                \textbf{0.85} &  0.51 &                  0.0 &  \textbf{0.02} & 0.42 &  \textbf{0.47}&         0.08 &  \textbf{0.26} &         0.14 &  \textbf{0.35} &          \textbf{0.82} &  0.91 &               0.58 &  \textbf{0.20} &           0.83 &  \textbf{0.21} \\
LRP-$\varepsilon$+   &                \textbf{0.63} &  0.57 &                  0.0 &  \textbf{0.01} & \textbf{0.30} &  0.27&        \textbf{0.24} &  0.21 &         \textbf{0.27} &  0.25 &          \textbf{0.34} &  0.39 &               0.62 &  \textbf{0.52} &           0.94 &  \textbf{0.60} \\
LRP-$\alpha2\beta1$ &                \textbf{0.82} &  0.67 &                  0.0 &  0.00 &  0.33 &  0.33&       0.22 &  \textbf{0.23} &         0.24 &  0.24 &          0.32 &  \textbf{0.28} &               0.63 &  \textbf{0.53} &           1.05 &  \textbf{0.61} \\
\bottomrule
\end{tabular}}

==> results/VOC/efb0_old.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &       0.54 &  \textbf{0.67} &                 0.00 &  0.00 &           0.06 &  \textbf{0.08} &         0.25 &  \textbf{0.34} &         0.29 &  \textbf{0.38} &          1.00 &  1.00 &            0.44 &  \textbf{0.36} &            0.49 &  \textbf{0.40} \\
LRP-$\varepsilon$+   &       0.52 &  \textbf{0.71} &                 0.01 &  0.01 &           0.05 &  0.05 &         0.27 &  \textbf{0.35} &         0.34 &  \textbf{0.38} &          \textbf{0.44} &  0.43 &            0.46 &  0.46 &            \textbf{0.52} &  0.53 \\
LRP-$\alpha2\beta1$ &       0.71 &  \textbf{0.75} &                 0.00 &  0.00 &           0.07 &  0.07 &         \textbf{0.32} &  0.31 &         \textbf{0.34} &  0.31 &          \textbf{0.43} &  0.36 &            0.58 &  0.58 &            \textbf{0.63} &  0.65 \\
\bottomrule
\end{tabular}}

==> results/VOC/efb4_old.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                0.68 &  \textbf{0.76} &                  0.0 &  0.0 & 0.02 & 0.02        & 0.30 &  \textbf{0.34} &         0.33 &  \textbf{0.35} &          \textbf{0.98} &  0.99 &               0.38 &  0.38 &           0.47 &  0.47 \\
LRP-$\varepsilon$+   &                0.55 &  \textbf{0.75} &                  0.0 &  0.0 &    0.00 & \textbf{0.01} &     0.18 &  \textbf{0.30} &         0.21 &  \textbf{0.32} &          0.51 &  \textbf{0.41} &               \textbf{0.43} &  0.49 &           \textbf{0.52} &  0.60 \\
LRP-$\alpha2\beta1$ &                0.71 &  \textbf{0.74} &                  0.0 &  0.0 & 0.02 & 0.02 &        0.17 &  \textbf{0.21} &         0.20 &  \textbf{0.23} &          0.40 &  \textbf{0.34} &               0.64 &  \textbf{0.62} &           \textbf{0.71} &  0.75 \\
\bottomrule
\end{tabular}}

==> results/VOC/reg18_old.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                0.50 &  \textbf{0.55} &                 0.01 &  0.01 & 0.29 & 0.29 &        0.29 &  \textbf{0.30} &         0.36 &  \textbf{0.37} &          \textbf{0.99} &  1.00 &               0.17 &  \textbf{0.15 }&           0.18 &  \textbf{0.15} \\
LRP-$\varepsilon$+  &                0.52 &  \textbf{0.58} &                 0.00 &  0.00 &    0.18 & 0.18 &     0.25 &  \textbf{0.28} &         0.30 &  \textbf{0.33} &          0.66 &  \textbf{0.64} &               \textbf{0.44} &  0.45 &           \textbf{0.59} &  0.60 \\
LRP-$\alpha2\beta1$ &                0.67 &  \textbf{0.74} &                 \textbf{0.01} &  0.00 &    0.18 & \textbf{0.23}&     0.26 & \textbf{0.30} &         0.28 &  \textbf{0.30} &          0.62 &  \textbf{0.56} &               \textbf{0.47} &  0.48 &           \textbf{0.59} &  0.60 \\
\bottomrule
\end{tabular}}

==> results/VOC/res50_old.tex <==
\resizebox{\textwidth}{!}{ \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                0.52 &  \textbf{0.60} &                  0.0 &  \textbf{0.01} &  0.37 & \textbf{0.39} &       0.28 &  \textbf{0.31} &         0.34 &  \textbf{0.37} &          1.00 &  1.00 &               0.19 &  \textbf{0.17} &           0.21 &  \textbf{0.18} \\
LRP-$\varepsilon$+   &                0.53 & \textbf{ 0.64} &                  0.0 &  0.00 & 0.19 & \textbf{0.20} &        0.25 &  \textbf{0.28} &         0.31 &  \textbf{0.32} &          0.67 &  \textbf{0.65} &               \textbf{0.47 }&  0.48 &           0.56 &  0.56 \\
LRP-$\alpha2\beta1$ &                0.68 &  \textbf{0.78} &                  0.0 &  0.00 &   0.37 & \textbf{0.42}&      0.26 &  \textbf{0.29} &         0.28 &  \textbf{0.29} &          0.63 &  \textbf{0.61} &               \textbf{0.49} &  0.51 &           \textbf{0.58} &  0.59 \\
\bottomrule
\end{tabular}}

==> results/VOC/vgg_old.tex <==
\resizebox{\textwidth}{!}{ 
\setlength{\tabcolsep}{5pt}
    \begin{tabular}{l||cc|cccc|cccc|cc|cccc}
    \toprule
    {} & \multicolumn{2}{c|}{Complexity} & \multicolumn{4}{c|}{Faithfulness} & \multicolumn{4}{c|}{Localization} & \multicolumn{2}{c|}{Random.} & \multicolumn{4}{c}{Robustness} \\
    {} & \multicolumn{2}{c|}{Spars.} & \multicolumn{2}{c}{Corr.}& \multicolumn{2}{c|}{AoPC} & \multicolumn{2}{c}{RMA} & \multicolumn{2}{c|}{RRA} & \multicolumn{2}{c|}{Logit} & \multicolumn{2}{c}{Avg. Sens.} & \multicolumn{2}{c}{Max Sens.} \\
    canonized &                  no &   yes &                  no &   yes &                   no &   yes &           no &   yes &           no &   yes &           no &   yes &            no &   yes &                 no &   yes  \\
    \midrule
EB       &                0.56 &  \textbf{0.58} &                 0.00 &  \textbf{0.01} & 0.63 & 0.63&        0.32 & \textbf{0.33} &         0.39 &  0.39 &          1.00 &  1.00 &               0.23 &  \textbf{0.19} &           0.24 &  \textbf{0.20} \\
LRP-$\varepsilon$+   &                0.56 &  \textbf{0.65} &                 0.01 &  0.01 &  0.22 & 0.22 &       0.30 &  \textbf{0.34} &         0.37 &  \textbf{0.39} &          0.41 &  \textbf{0.38} &               \textbf{0.51} &  0.52 &           0.64 &  0.64 \\
LRP-$\alpha2\beta1$ &                0.72 &  \textbf{0.84} &                \textbf{0.01} &  0.00 & 0.41 & \textbf{0.50}&         0.31 &  \textbf{0.38} &         0.33 &  \textbf{0.36} &          \textbf{0.47} &  0.56 &              \textbf{ 0.53} &  0.54 &           0.65 &  0.65 \\
\bottomrule
\end{tabular}
}

==> results/clevr_xai_pos_sq_sum.tex <==
\resizebox{\textwidth}{!}{ \begin{tabular}{l||l|rr|rr|rr|rr|rr|rr}
\toprule
{}& {} & \multicolumn{2}{l|}{$\uparrow$ Complexity} & \multicolumn{2}{l|}{$\uparrow$ Faithfulness} & \multicolumn{2}{l|}{$\uparrow$ Local. (RRA)} & \multicolumn{2}{l|}{$\uparrow$ Local. (RMA)} & \multicolumn{2}{l|}{$\downarrow$ Robustness} & \multicolumn{2}{l}{$\downarrow$ Random.} \\
Questions & canonized &         no &   yes &           no &   yes &           no &   yes &           no &   yes &          no &   yes &            no &   yes \\
\midrule
% \multirow{8}{*}{Simple} & Saliency   &       0.97 &  0.97 &         0.72 &  0.72 &         0.26 &  0.26 &         0.37 &  0.37 &        0.02 &  0.02 &          0.97 &  0.97 \\
% & Smoothgrad &       0.94 &  0.94 &         0.72 &  0.72 &         0.35 &  0.35 &         0.46 &  0.46 &        0.02 &  0.02 &          0.96 &  0.96 \\
% & IG         &       0.99 &  0.95 &         0.75 &  0.75 &         \textbf{0.41} &  0.20 &         \textbf{0.70} &  0.27 &        0.02 &  0.02 &          0.98 &  \textbf{0.96} \\
% & GB         &       0.97 &  0.97 &         0.74 &  0.74 &         0.32 &  0.32 &         0.39 &  0.39 &        0.02 &  0.02 &          0.98 &  0.98 \\
% & EB         &       \textbf{0.99} &  0.97 &         0.72 &  0.72 &         0.57 &  \textbf{0.61} &         0.68 &  \textbf{0.70} &        \textbf{0.02} &  0.03 &          1.00 &  1.00 \\
% & LRP-EP     &       0.98 &  0.98 &         0.63 &  \textbf{0.64} &         \textbf{0.47} &  0.45 &         \textbf{0.60} &  0.57 &        0.03 &  \textbf{0.02} &          0.98 &  0.98 \\
% & LRP-a2b1   &       \textbf{0.98} &  0.97 &         0.71 &  \textbf{0.72} &         \textbf{0.47} &  0.37 &         \textbf{0.64} &  0.52 &        0.02 &  0.02 &          0.99 &  \textbf{0.98} \\
% & LRP-Leila  &       0.95 &  \textbf{0.98} &         0.71 &  \textbf{0.72} &         0.70 &  0.70 &         0.75 &  \textbf{0.82} &        0.03 &  0.03 &          1.00 &  1.00 \\

\midrule
\multirow{4}{*}{Simple} & EB        &       0.99 &  0.97 &         0.71 &  0.72 &         0.62 &  0.60 &         0.75 &  0.68 &        1.43 &  1.41 &    1.00 &  1.00 \\
& LRP-$\varepsilon+$    &       0.98 &  0.98 &         0.66 &  0.64 &         0.45 &  0.44 &         0.57 &  0.56 &        1.49 &  1.50 &    0.87 &  0.88 \\
& LRP-$\alpha2\beta1$  &       0.98 &  0.97 &         0.71 &  0.74 &         0.46 &  0.36 &         0.63 &  0.50 &        1.50 &  1.50 &    0.86 &  0.81 \\
& LRP-Leila &       0.95 &  0.98 &         0.72 &  0.71 &         0.70 &  0.69 &         0.75 &  0.82 &        1.37 &  1.40 &    0.99 &  1.00 \\

\midrule


% \multirow{8}{*}{Complex} & Saliency   &       0.96 &  0.96 &         0.64 &  0.64 &         0.28 &  0.28 &         0.45 &  0.45 &        0.02 &  0.02 &          0.96 &  0.96 \\
% & Smoothgrad &       0.92 &  0.92 &         0.63 &  0.63 &         0.27 &  0.27 &         0.45 &  0.45 &        0.03 &  0.03 &          0.93 &  0.93 \\
% & IG         &       \textbf{0.99} &  0.93 &         \textbf{0.67} &  0.66 &         \textbf{0.49} &  0.17 &         \textbf{0.85} &  0.26 &        \textbf{0.02} &  0.03 &          0.98 &  \textbf{0.93} \\
% & GB         &       0.97 &  0.97 &         0.65 &  0.65 &         0.33 &  0.33 &         0.47 &  0.47 &        0.02 &  0.02 &          0.97 &  0.97 \\
% & EB         &       \textbf{0.99} &  0.96 &         0.64 &  \textbf{0.65} &         \textbf{0.65} &  0.62 &         \textbf{0.78} &  0.77 &        0.02 &  0.02 &          1.00 &  1.00 \\
% & LRP-EP     &       0.97 &  \textbf{0.98} &         0.55 &  \textbf{0.56} &         0.35 &  \textbf{0.42} &         0.67 &  \textbf{0.72} &        0.03 &  \textbf{0.02} &          \textbf{0.97} &  0.98 \\
% & LRP-a2b1   &       \textbf{0.97} &  0.96 &         \textbf{0.64} &  0.63 &         \textbf{0.44} &  0.37 &         \textbf{0.72} &  0.60 &        0.02 &  0.02 &          0.98 &  0.98 \\
% & LRP-Leila  &       0.94 &  \textbf{0.97} &         0.64 &  \textbf{0.65} &         0.54 &  \textbf{0.63} &         0.79 &  \textbf{0.86} &        0.03 &  0.03 &          1.00 &  1.00 \\
% \midrule
\multirow{3}{*}{Complex} & EB        &       0.99 &  0.97 &         0.64 &  0.65 &         0.65 &  0.61 &         0.82 &  0.77 &        1.39 &  1.36 &    1.00 &  0.99 \\
& LRP-$\varepsilon+$    &       0.97 &  0.98 &         0.54 &  0.55 &         0.34 &  0.40 &         0.65 &  0.71 &        1.50 &  1.49 &    0.85 &  0.87 \\
& LRP-$\alpha2\beta1$  &       0.97 &  0.96 &         0.63 &  0.63 &         0.43 &  0.37 &         0.71 &  0.60 &        1.50 &  1.50 &    0.80 &  0.75 \\
& LRP-Leila &       0.94 &  0.97 &         0.64 &  0.64 &         0.54 &  0.63 &         0.79 &  0.86 &        1.36 &  1.38 &    0.98 &  0.99 \\

\bottomrule
\end{tabular}
}

==> results/clevr_xai_sum.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{l||l|rr|rr|rr|rr|rr|rr}
\toprule
{}& {} & \multicolumn{2}{l|}{Complexity} & \multicolumn{2}{l|}{Faithfulness} & \multicolumn{2}{l|}{Local. (RRA)} & \multicolumn{2}{l|}{Local. (RMA)} & \multicolumn{2}{l|}{Robustness} & \multicolumn{2}{l}{Random.} \\
Questions & canonized &         no &   yes &           no &   yes &           no &   yes &           no &   yes &          no &   yes &            no &   yes \\
\midrule
\multirow{4}{*}{Simple} 
& EB        &       \textbf{0.96} &  0.87 &         0.71 &  \textbf{0.72} &         \textbf{0.61} &  0.59 &         \textbf{0.64} &  0.50 &        1.40 &  \textbf{1.35} &    1.00 &  1.00 \\
% & LRP-$\varepsilon+$                    &       0.81 &  \textbf{0.89} &         0.64 &  0.64 &         0.42 &  \textbf{0.46} &         0.36 &  \textbf{0.43} &        \textbf{1.52} &  1.53 &    \textbf{0.71} &  0.72 \\
% & LRP-$\alpha2\beta1$               &       0.82 &  \textbf{0.84} &         \textbf{0.71} &  0.69 &         \textbf{0.43} &  0.34 &         \textbf{0.40} &  0.33 &        1.54 &  1.54 &    0.68 &  \textbf{0.66} \\
& LRP-Custom                         &       0.82 &  \textbf{0.90} &         0.72 &  0.72 &         \textbf{0.70} &  0.69 &         0.53 &  \textbf{0.63} &        \textbf{1.28} &  1.33 &    0.99 &  0.99 \\

& EB        &       0.99 &  0.97 &         0.50 &  0.51 &         0.64 &  0.61 &         0.76 &  0.70 &        1.37 &  1.39 &    1.00 &  1.0 \\
& LRP-Leila &       0.95 &  0.98 &         0.52 &  0.52 &         0.70 &  0.70 &         0.75 &  0.83 &        1.33 &  1.35 &    0.99 &  1.0 \\

\midrule
\multirow{4}{*}{Complex} & EB        &       \textbf{0.96} &  0.87 &         0.64 &  \textbf{0.65} &         \textbf{0.64} &  0.60 &         \textbf{0.76} &  0.65 &        1.36 &  \textbf{1.30} &    1.00 &  \textbf{0.99} \\
% & LRP-$\varepsilon+$                   &       0.80 &  \textbf{0.88} &         0.53 &  \textbf{0.55} &         0.32 &  \textbf{0.46} &         0.46 &  \textbf{0.60} &        1.53 &  1.53 &    \textbf{0.65} &  0.69 \\
% & LRP-$\alpha2\beta1$               &       0.81 &  \textbf{0.82} &         0.63 &  0.63 &         \textbf{0.38} &  0.34 &         \textbf{0.50} &  0.44 &        \textbf{1.53} &  1.54 &    0.61 &  \textbf{0.59} \\
& LRP-Custom                         &       0.82 &  \textbf{0.90} &         0.64 &  0.64 &         0.54 &  \textbf{0.62} &         0.63 &  \textbf{0.74} &        \textbf{1.26} &  1.29 &    \textbf{0.98} &  0.99 \\



\bottomrule
\end{tabular}
}
